Uncovering the Portability Limitation of Deep Learning-Based Wireless Device Fingerprints

Recent device fingerprinting approaches rely on deep learning to extract device-specific features solely from raw RF signals to identify, classify and authenticate wireless devices. One widely known issue lies in the inability of these approaches to maintain good performances when the training data and testing data are collected under varying deployment domains. For example, when the learning model is trained on data collected from one receiver but tested on data collected from a different receiver, the performance degrades substantially compared to when both training and testing data are collected using the same receiver. The same also happens when considering other varying domains, like channel condition and protocol configuration. In this paper, we begin by explaining, through testbed experiments, the challenges these fingerprinting techniques face when it comes to domain portability. We will then present some ideas on how to go about addressing these challenges so as to make deep learning-based device fingerprinting more resilient to domain variability.

==> 8-acknowledgement.tex <==
This research is supported in part by the National Science Foundation and Intel under Award No. 2003273.  
We would like to thank Intel researchers, Dr. Kathiravetpillai Sivanesan, Dr. Lily Yang, Dr. Richard Dorrance, and Dr. Vesh Raj Sharma Banjade, for their constructive feedback. 

